Nuclear Atomic Norm for parametric estimation of sparse channels

Parametric channel estimation in mmWave not only enables the anticipated large spectral efficiency gains of \acs{MIMO} systems but also reveals important propagation parameters, allowing for a low complexity representation of the channel matrix. In this work, we propose to use atomic norm as a gridless multidimensional spectral estimation approach to address parametric channel estimation where both AoD and AoA are identified. The conditions for recovery of the propagation parameters are given depending on properties of the measurement matrix, and on structural features such as the antenna geometry or the number of scatters to resolve. The proposed methodology is compared against several state-of-the-art parametric approaches.

==> App2_long.tex <==
We start the proof by recalling that the fact that matrix $\miT_\TT\in\C^{\Tu\times\Tu}$ with $\rank$ $r_1<\Tsf_{\ddl}$  belongs to the set of \ac{PSD} canonical $\ddl$-\ac{MLT} matrices $\mathcal{T}^{\ddl}_\TT$, means that it has a multi-level Toeplitz matrix structure as in Definition \ref{definitionMLT} and the \emph{dimension vector} $\TT=[\Tsf_1,\Tsf_2,\dots,\Tsf_{\ddl}]$ has an ordering such that $\Tsf_1 \leq \Tsf_2\leq\dots \leq\Tsf_{\ddl}$ with $\Tu=\prod_{i=1}^{\ddl}\Tsf_i$. Furthermore, for $1\leq t\leq\ddl$, we recall that the (sub)matrix nested along the left upper block diagonal\footnote{$\miT_{\mathbf{0}\TT_{t:\ddl}}$ is the $\prod_{i=t}^{\ddl}\Tsf_i\times\prod_{i=t}^{\ddl}\Tsf_i$ subblock of $\miT_\TT$ obtained considering the first $\prod_{i=t}^{\ddl}\Tsf_i$ rows and the first $\prod_{i=t}^{\ddl}\Tsf_i$ columns of $\miT_\TT$. } $\miT_{\mathbf{0}\TT_{t:\ddl}}\in\C^{\prod_{i=t}^{\ddl}\Tsf_i\times\prod_{i=t}^{\ddl}\Tsf_i}$ is a  $(\ddl-t-1)$-\ac{MLT} matrix % where $[\mathbf{0}\TT_{t:\ddl}]=[\underbrace{0,\dots,0}_{t-1}\TT_{t:\ddl}]$. 
and we set  $r_t=\rank\left\{\miT_{\mathbf{0}\TT_{t:\ddl}}\right\}$. 
From \cite[Thm. 4.1]{Meyer73} we have that $r_{\ddl}\leq r_{\ddl-1}\leq\dots\leq r_{1} $ and therefore $r_{\ddl}\leq r_{\ddl-1}\leq\dots\leq r_{1} <\Tsf_{\ddl}$.
%\begin{equation}
%\label{inequlity}
%r_{\ddl}\leq r_{\ddl-1}\leq\dots\leq r_{1} <\Tsf_{\ddl}
%\end{equation}
By \cite[Lemma in Proposition 1]{Gurvits_prueba} we have that, if $r_t<\prod_{i=t+1}^{\ddl}\Tsf_i$,  a \ac{PSD} block matrix $\miT_{\mathbf{0}\TT_{t:\ddl}}$ is decomposed as:
$$
\miT_{\mathbf{0}\TT_{t:\ddl}}=\sum_{j=1}^{r_t} 
(\miu_{\Tsf_t}(\nu^t_j)\otimes  \mig^{t+1}_{j})(\miu_{\Tsf_t}(\nu^t_j)\otimes  \mig^{t+1}_{j})^\H=\miC_{t:\ddl} \miC_{t:\ddl}^\H
$$
where $\nu^t_j\in \T$, with $j \in [r_t]$ and $\miC_{t:\ddl}\in\C^{\prod_{i=t}^{\ddl}\Tsf_i\times r_t}$ can be also written as:
\begin{eqnarray}
\miC_{t:\ddl}&=&[\mic^t_1,..,\mic^t_{r_t} ]=[\miu_{\Tsf_t}(\nu^t_1)\otimes  \mig^{t+1}_{1},..,\miu_{\Tsf_t}(\nu^t_{r_t})\otimes  \mig^{t+1}_{r_t}] \nonumber\\
&=&\miU_{\Tsf_t}(\ll^{t}_{1:r_t}) \odot \miG_{t+1:\ddl}.\nonumber
\label{machec0}
\end{eqnarray}

Also denoting $\miT_{\mathbf{0}\a\TT_{t+1:\ddl}}$ as the $\a$-th block of $\miT_{\mathbf{0}\TT_{t:\ddl}}$ for  $-\Tsf_t+1\leq \a\leq\Tsf_t-1$ we have that
\begin{eqnarray}
\miT_{\mathbf{0}\a\TT_{t+1:\ddl}}&=&\sum_{j=1}^{r_t} e^{\j2\pi \a \nu^{t}_j}  \mig^{t}_{j} \mig^{t\H}_{j}\label{incredibile00}\\
&=&\miG_{t+1:\ddl}\diag(e^{\j2\pi\a \nu^{t}_1}, \ldots, e^{\j2\pi\a \nu^{t}_{r_t}})\miG_{t+1:\ddl}^\H
\nonumber\\
&=&\miG_{t+1:\ddl}\miD_t^\a\miG_{t+1:\ddl}^\H
\nonumber
\end{eqnarray}
with $\miD_t= \diag(e^{\j2\pi \nu^{t}_1}, \ldots, e^{\j2\pi \nu^{t}_{r_t}})$. Similarly, we have:
\begin{eqnarray}
\miT_{\mathbf{0}\TT_{t+1:\ddl}}&=&\sum_{j=1}^{r_{t+1}} 
(\miu_{\Tsf_{t+1}}(\nu^{t+1}_j)\otimes  \mig^{t+2}_{j})(\miu_{\Tsf_{t+1}}(\nu^{t+1}_j)\otimes  \mig^{t+2}_{j})^\H\nonumber\\&=&\miC_{t+1:\ddl} \miC_{t+1:\ddl}^\H
\nonumber
\end{eqnarray}

Setting $\a=0$ in \eqref{incredibile00}, we necessarily have that $\miG_{t+1:\ddl}\miG_{t+1:\ddl}^\H=\miC_{t+1:\ddl} \miC_{t+1:\ddl}^\H$ and therefore, we can always find  a $r_{t+1}\times r_{t}$ unitary matrix, $\miO_t$, such that 
\begin{eqnarray}
\miG_{t+1:\ddl}=\miC_{t+1:\ddl}\miO_{t}
\label{musica}
\end{eqnarray}

Given this, for $j\in[r_t]$ and $t\leq\ddl-2$ we have: 
\begin{equation}
\begin{split}
\mic_j^{t}&=\miu_{\Tsf_t}(\nu^{t}_j) \otimes\sum_{i=1}^{r_{t+1}}o^{t}_{ji}\miu_{\Tsf_{t+1}}(\nu^{t+1}_i) \otimes\mig^{t+2}_{i}\end{split}
\label{cxyz}
\end{equation}
where $o^{t}_{ji}$ is the element in row $j$ and column $i$ of matrix $\miO_{t}$.

Applying recursively the relationship in \eqref{musica} and following the structure in \eqref{cxyz}, for $t=1$, i.e. for $\miT_\TT=\miC_{1:\ddl} \miC_{1:\ddl}^\H$, and $i_1=[r_1]$ we have:
\begin{equation}
\begin{split}
\mic_{i_1}^{1}&=\miu_{\Tsf_1}(\nu^{1}_{i_1}) \otimes\sum_{i_2=1}^{r_{2}}o^{2}_{i_2i_1}\miu_{\Tsf_{2}}(\nu^{2}_{i_2}) \otimes\dots\\&\dots\otimes\sum_{i_{\ddl}=1}^{r_{\ddl}}o^{\ddl}_{i_{\ddl}i_{\ddl-1}}p_{i_{\ddl}}\miu_{\Tsf_{\ddl}}(\nu^{\ddl}_{i_{\ddl}})\\
&=\sum_{i_2=1}^{r_{2}}\dots\sum_{i_{\ddl}=1}^{r_{\ddl}}p_{i_{\ddl}}\Motimes_{s=1}^{\ddl}o^{s}_{i_{s}i_{s-1}}\miu_{\Tsf_s}(\nu^{s}_{i_s}) \\
%&=\sum_{i_2=1}^{r_{2}}\dots\sum_{i_{\ddl}=1}^{r_{\ddl}}p_{i_{\ddl}}\prod_{m=2}^{\ddl} o^{m}_{i_{\ddl}i_{\ddl-1}} \Motimes_{l=1}^{\ddl}\miu_{\TT}(\ell^{l}_{i_l}) 
\end{split}
\label{Cxyz}
\end{equation}
where $p_{i_{\ddl}}$ with $i_{\ddl}\in[r_{\ddl}]$ are the elements of the diagonal of the Vandermonde decomposition of the Toeplitz matrix $\miT_{\mathbf{0}\Tsf_{\ddl}}$ found in the very last nesting and we define $o^{1}_{i_{1}i_{0}}=1$.

The column elements of $\miC_{1:\ddl}=[\mic_{1}^{1},\dots,\mic_{r_1}^{1}]$ described in \eqref{Cxyz} are generated by $\prod_{s=1}^{\ddl}r_s$ vectors $\Motimes_{s=1}^{\ddl}\miu_{\Tsf_s}(\nu^{s}_{i_s}) $ with $i_s\in[r_s]$, which necessarily need to be linearly dependent given that $\rank\{\miT_\TT\}=\rank\{\miC_{1:\ddl}\miC_{1:\ddl}^\H\}=r_1$. We define $\mathcal{M}$ as the set of indexes $(i_{1,m},\dots,i_{\ddl,m})$ such that the vectors  $\Motimes_{s=1}^{\ddl}\miu_{\Tsf_s}(\nu^{s}_{i_{s,m}})$ are linearly independent, note that $|\mathcal{M}|=r_1$ and $m\in[r_1]$. Then, the linearly independent generating vectors of matrix $\miC_{1:\ddl}$, now indexed in $m\in[r_1]$, are $\Motimes_{s=1}^{\ddl}\miu_{\Tsf_s}(\nu^{s}_{i_{s,m}})=\miu_\TT(\ll_m)$ where $\ll_m=[\nu^{1}_{i_{1,m}},\dots,\nu^{\ddl}_{i_{\ddl,m}}]^\top$.

Due to Schur complement lemma, the model $\mil_u$ that satisfies constraint $\begin{bmatrix}\miT_{\TT} &\mil_u\\ \mil_u^\H & l\end{bmatrix}\succeq 0$ also satisfies $\miT_{\TT} -( l)^{-1}\mil_u\mil_u^\H\succeq 0$ which implies that $\mil_u\in\spn\{\miT_{\TT}\}=\spn\{\miC_{1:\ddl}\miC_{1:\ddl}^\H\}$. Therefore there exist two set of coefficients $[\alpha_1, \ldots, \alpha_{r_1}]$ and $[\beta_1, \ldots, \beta_{r_1}]$ such that 
\begin{eqnarray}
\mil_u&=&\sum_{k=1}^{r_1}\alpha_k\mic_{k}^{1}
=\sum_{i_1=1}^{r_1}\dots\sum_{i_{\ddl}=1}^{r_{\ddl}}\alpha_{i_1}p_{i_{\ddl}}\Motimes_{s=1}^{\ddl}o^{s}_{i_{s}i_{s-1}}\miu_{\Tsf_s}(\nu^{s}_{i_s})\nonumber\\
&=&\sum_{k=1}^{r_1}\beta_k\miu_\TT\left(\ll_{k}\right)
\label{decomp}
\end{eqnarray}
%Recall that in this work we restrict our analysis to those scenarios where the sparsity condition $\Tu \gg \K$ conveys to  $\Tu > 2\K$ and the measurement scenario to $\Ta>2\K$. We show the proof next for a set of frequencies $\ff_{1:\K}$ under  A.\ref{A1} and $\ll_{1:r}$ any arbitrary set in $\T^{\ddl\times r}$. By assumption we also have that $\Tu > 2r$ and  $\Ta>2r$.


==> Change.tex <==
{\RED ANTONIA, WE USE LEMMA 2 TO PROOF THIS THM. (following  what we did in the Gridless paper). TO USE LEMMA 2, WE NEED THAT $\K<\Tsf_{\ddl}$ or that $\rank\{\miT^\opt_{\TT}\}<\Tsf_{\ddl}$, THEREFORE WE ALSO NEED $\K<\Tsf_{\ddl}$ FOR THE UNIQUENESS OF THE SPARSE VECTOR, NOT ONLY FOR THE FREQUENCY RECOVERY, THAT IS WHY I HAVE REPHRASED. WE CAN GO BACK TO YOUR VERSION, BUT THEN WE NEED TO DISCUSS HOW TO PROOF...

SAME THING APPLIES TO THM. USING THE TRACE.
}

==> figures/freqs_error_pilots_noiseless_comparison_wrt_k_all_P_1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\pgfplotsset{
    legend image with text/.style={
        legend image code/.code={%
            \node[anchor=center] at (0.3cm,0cm) {#1};
        }
    },
}



\begin{tikzpicture}

\begin{axis}[%
width=0.8\figurewidth,
height=0.8\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=1,
xmax=6,
xlabel style={font=\color{white!15!black}},
xlabel={K},
ymode=log,
ymin=0.0125547379079762,
ymax=0.047112180087017,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\error$},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
% yminorgrids,
legend columns=4, 
legend style={
            % the /tikz/ prefix is necessary here...
            % otherwise, it might end-up with `/pgfplots/column 2`
            % which is not what we want. compare pgfmanual.pdf
    /tikz/column 5/.style={
        column sep=5pt,
    },
},
legend style={at={(0.0,1.5)}, anchor=north west, legend cell align=left, align=left, draw=none}
]

\addlegendimage{legend image with text={\tiny \randc{} }}
\addlegendentry{}
\addlegendimage{legend image with text={\tiny \rand{} }}
\addlegendentry{}
\addlegendimage{legend image with text={\tiny \binc{} }}
\addlegendentry{}
\addlegendimage{legend image with text={\tiny \bin{} }}
\addlegendentry{}




\addplot [color=blue, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, blue}]
  table[row sep=crcr]{%
1	0.033378038185992\\
2	0.033190738984751\\
3	0.0334638626996523\\
4	0.0345226127924874\\
5	0.0354155705724105\\
6	0.0392150797653575\\
};
\addlegendentry{}

\addplot [color=red, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, red}]
  table[row sep=crcr]{%
1	0.047112180087017\\
2	0.0275981942571692\\
3	0.0294808992147464\\
4	0.0303880565869905\\
5	0.0309612452218698\\
6	0.0331565502726694\\
};
\addlegendentry{}

\addplot [color=green, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, green}]
  table[row sep=crcr]{%
1	0.0241323558150568\\
2	0.0214828283099366\\
3	0.0225611343293181\\
4	0.0229924330075814\\
5	0.0239026153390115\\
6	0.0278982281292516\\
};
\addlegendentry{}

\addplot [color=black, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, black}]
  table[row sep=crcr]{%
1	0.0125547379079762\\
2	0.0233225159074661\\
3	0.0199914458932555\\
4	0.0195813831094757\\
5	0.0214690756829905\\
6	0.0249147706874427\\
};
\addlegendentry{\tiny $\P=1$}

\end{axis}
\end{tikzpicture}%

==> figures/freqs_error_pilots_noiseless_comparison_wrt_k_all_P_200.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{
    legend image with text/.style={
        legend image code/.code={%
            \node[anchor=center] at (0.3cm,0cm) {#1};
        }
    },
}



\begin{tikzpicture}

\begin{axis}[%
width=0.8\figurewidth,
height=0.8\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=1,
xmax=6,
xlabel style={font=\color{white!15!black}},
xlabel={K},
ymode=log,
ymin=1e-6,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\error$},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
% yminorgrids,
legend columns=4, 
legend style={
            % the /tikz/ prefix is necessary here...
            % otherwise, it might end-up with `/pgfplots/column 2`
            % which is not what we want. compare pgfmanual.pdf
    /tikz/column 5/.style={
        column sep=5pt,
    },
},
legend style={at={(0.0,1.5)}, anchor=north west, legend cell align=left, align=left, draw=none}
]

\addlegendimage{legend image with text={\tiny \randc{} }}
\addlegendentry{}
\addlegendimage{legend image with text={\tiny \rand{} }}
\addlegendentry{}
\addlegendimage{legend image with text={\tiny \binc{} }}
\addlegendentry{}
\addlegendimage{legend image with text={\tiny \bin{} }}
\addlegendentry{}

\addplot [color=blue, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, blue}]
  table[row sep=crcr]{%
1	0.00399493748014461\\
2	0.00397525368751721\\
3	0.00350131127159696\\
4	0.00381178619020987\\
5	0.0040362986218828\\
6	0.00843392768831972\\
};
\addlegendentry{}

\addplot [color=red, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, red}]
  table[row sep=crcr]{%
1	1.70152730647013e-08\\
2	0.000416248698650917\\
3	0.000366682438535304\\
4	0.000688247016424915\\
5	0.000913383948421801\\
6	0.00580989704676381\\
};
\addlegendentry{}

\addplot [color=green, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, green}]
  table[row sep=crcr]{%
1	0.00239379038505885\\
2	0.0021379297389847\\
3	0.00241392655303151\\
4	0.00286068940184607\\
5	0.00284130571366879\\
6	0.00802641376947517\\
};
\addlegendentry{}

\addplot [color=black, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, black}]
  table[row sep=crcr]{%
1	0.00733883553847041\\
2	0.00730923637976778\\
3	0.00717653962454023\\
4	0.00754737733770641\\
5	0.00835442970686604\\
6	0.0130775216997484\\
};
\addlegendentry{\tiny $\P=3$}

\addplot [color=blue, dashed, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, blue}]
  table[row sep=crcr]{%
1	1.47984486439987e-21\\
2	3.66572687790477e-06\\
3	2.5693552076086e-06\\
4	6.2222451605952e-06\\
5	4.68926207569523e-05\\
6	0.00514356623774117\\
};
\addlegendentry{}

\addplot [color=red, dashed, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, red}]
  table[row sep=crcr]{%
1	1.46639578643464e-21\\
2	3.66515530166747e-06\\
3	2.56936900800893e-06\\
4	6.22231754049253e-06\\
5	4.68925232321784e-05\\
6	0.00421692101506695\\
};
\addlegendentry{}

\addplot [color=green, dashed, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, green}]
  table[row sep=crcr]{%
1	9.19742155547947e-20\\
2	1.01971229303748e-05\\
3	9.21384976910314e-06\\
4	1.2078426206759e-05\\
5	0.000106199035627623\\
6	0.00530032399348339\\
};
\addlegendentry{}

\addplot [color=black, dashed, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, black}]
  table[row sep=crcr]{%
1	0.00438373246157964\\
2	0.0041565323106285\\
3	0.00436769381153895\\
4	0.00472439935532956\\
5	0.00528865049408505\\
6	0.00982531789458726\\
};
\addlegendentry{\tiny $\P=4$}

\addplot [color=blue, dotted, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, blue}]
  table[row sep=crcr]{%
1	1.25064948111542e-21\\
2	3.6638393352883e-06\\
3	2.56907699256133e-06\\
4	6.22184609973911e-06\\
5	4.68935337647113e-05\\
6	0.00472019282667306\\
};
\addlegendentry{}

\addplot [color=red, dotted, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, red}]
  table[row sep=crcr]{%
1	2.56327250072743e-21\\
2	3.66372858190806e-06\\
3	2.56915601140847e-06\\
4	6.22207087508726e-06\\
5	4.68924578411306e-05\\
6	0.00441356087567894\\
};
\addlegendentry{}

\addplot [color=green, dotted, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, green}]
  table[row sep=crcr]{%
1	2.1849056545442e-21\\
2	3.66396872068107e-06\\
3	2.56913228402431e-06\\
4	6.22207390279204e-06\\
5	4.68933741310277e-05\\
6	0.00434047574787196\\
};
\addlegendentry{}

\addplot [color=black, dotted, line width=1.0pt, mark=triangle, mark options={solid, rotate=180, black}]
  table[row sep=crcr]{%
1	0.00187338286674627\\
2	0.00153003193313843\\
3	0.00161439169755802\\
4	0.00158361220161311\\
5	0.0017807017594024\\
6	0.00696499366564277\\
};
\addlegendentry{\tiny $\P=6$}

\end{axis}
\end{tikzpicture}%
